The 4th Reactive Synthesis Competition (SYNTCOMP 2017): Benchmarks, Participants & Results

We report on the fourth reactive synthesis competition (SYNTCOMP 2017). We introduce two new benchmark classes that have been added to the SYNTCOMP library, and briefly describe the benchmark selection, evaluation scheme and the experimental setup of SYNTCOMP 2017. We present the participants of SYNTCOMP 2017, with a focus on changes with respect to the previous years and on the two completely new tools that have entered the competition. Finally, we present and analyze the results of our experimental evaluation, including a ranking of tools with respect to quantity and quality of solutions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{116}
\providecommand{\publicationstatus}{D. Fisman, S. Jacobs (Eds.): Sixth Workshop on Synthesis (SYNT 2017)\\
EPTCS 260, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.260.10}{10.4204/EPTCS.260.10}}
\pdfoutput=1


==> rules.tex <==
\section{Synthesis Problem (TODO)}
\label{sec:problem}

We briefly summarize the reactive synthesis problem as it is considered in \syntcomp. A more detailed introduction into the problem, as well as into the different approaches for solving it, can be found in~\cite{SYNTCOMP14}.

In \syntcomp, we consider the automatic synthesis of finite-state reactive systems that satisfy a safety specification, given as a monitor circuit that raises a special output \out when an unsafe state is visited. The specification is encoded in the \syntcomp format, an extension of the well-known AIGER format~\cite{aiger} that allows inputs of the circuit to be defined as either controllable or uncontrollable. In the traditional game-based approach to the synthesis of reactive systems~\cite{BL69,Rabin69,Thomas95}, such a specification gives rise to a \emph{game }between
two players: states of the game are given by the valuation of latches in the monitor circuit, the environment player decides on the uncontrollable inputs of the specification circuit, and the system player decides on the controllable inputs. The goal of the system player is to satisfy
the specification, i.e., to visit only safe states, independent of the environment
behavior.  

Algorithms that solve this game usually take an approach that consists of two steps. In the first step, a so-called \emph{winning region} is computed. The
winning region $W$ is the set of all states from which the system player can enforce
to satisfy the specification, i.e., to visit only safe states in the subsequent computation. In the classical algorithm, this is done by computing the fixpoint of the \emph{uncontrollable predecessor} operation \upre on the error states, i.e., inductively computing all states from which the environment can force the game into the unsafe states. Since two-player safety games are determined, the complement of this set is the winning region $W$ of the system player.
In a second step, a \emph{winning strategy} is derived from the
winning region.  For every (current) state and uncontrollable input, the winning strategy
defines a set of controllable inputs that are okay for satisfying the specification. In order to obtain an implementation of this strategy as a circuit, a concrete choice
for the controllable inputs has to be made for every state and uncontrollable input.

In order to achieve acceptable scalability, it is important to implement
synthesis algorithms symbolically, i.e., by manipulating formulas instead of
enumerating states. In synthesis, these symbolic algorithms are usually implemented with Binary Decision Diagrams (BDDs)~\cite{bryant86,somenzi99,AlurMN05}.  One reason for this is
that solving games inherently involves dealing with quantifier alternations,
% (for
% each input, there must exist some output such that a certain goal is achieved),
and BDDs offer techniques for handling both kinds of quantification. However, BDDs also have their
scalability issues.  
On the other hand, there have been enormous performance
improvements in decision procedures for the satisfiability of (boolean) formulas over the
last years and decades.  This has lead to efficient tools like SAT- and QBF
(Quantified Boolean Formulas) solvers, which can also be leveraged to obtain efficient symbolic synthesis algorithms.

All of the tools that compete in \syntcomp 2015 implement symbolic game-based synthesis in some form. A description of the tools will be given in Section~\ref{sec:participants}.
